Stochastic Games with Lexicographic Reachability-Safety Objectives

We study turn-based stochastic zero-sum games with lexicographic preferences over reachability and safety objectives. Stochastic games are standard models in control, verification, and synthesis of stochastic reactive systems that exhibit both randomness as well as angelic and demonic non-determinism. Lexicographic order allows to consider multiple objectives with a strict preference order over the satisfaction of the objectives. To the best of our knowledge, stochastic games with lexicographic objectives have not been studied before. We establish determinacy of such games and present strategy and computational complexity results. For strategy complexity, we show that lexicographically optimal strategies exist that are deterministic and memory is only required to remember the already satisfied and violated objectives. For a constant number of objectives, we show that the relevant decision problem is in NP $\cap$ coNP, matching the current known bound for single objectives; and in general the decision problem is PSPACE-hard and can be solved in NEXPTIME $\cap$ coNEXPTIME. We present an algorithm that computes the lexicographically optimal strategies via a reduction to computation of optimal strategies in a sequence of single-objectives games. We have implemented our algorithm and report experimental results on various case studies.

==> 5_robustness.tex <==
\section{Assessing Strategy Robustness}
\label{sec:robust}

\todo[inline]{This section is not polished yet; not sure yet whether to polish and keep or to drop, depending on time}

Lex-optimal strategies generally lack \emph{robustness} against changes in the opponents counter-stratey. In fact, it is possible that a counter-strategy that is not lex-optimal grants an arbitrarily small gain in some objective $i < n$ while causing a maximal decrease in another objective $j > i$:

\begin{figure}
	\centering
\begin{subfigure}{0.75\textwidth}


\begin{tikzpicture}[on grid,node distance=12mm and 15mm]
	\node[max] (s_0) {$s_0$};
	\node[min,left=of s_0] (s_1) {$s_1$};
	\node[min,right=of s_0] (s_2) {$s_2$};
	\node[below=of s_0] (t_0) {$(0.5,1)$};
	\node[below=of s_1,xshift=-10mm] (t_1) {$(0.5 + \epsilon,0)$};
	\node[below=of s_2,xshift=10mm] (t_2) {$(1,0.5)$};
	
	\draw[trans] (s_0) -- (s_1);
	\draw[trans] (s_0) -- (s_2);
	\draw[trans] (s_1) edge[bend right=0] (t_1.north);
	\draw[trans] (s_2) -- (t_2.north);
	\draw[trans] (s_1) edge[bend right=0] (t_0);
	\draw[trans] (s_2) edge[bend left=0] (t_0);
\end{tikzpicture}
\subcaption{}
\end{subfigure}
\begin{subfigure}{0.24\textwidth}
\begin{tikzpicture}[scale=1.5]
	\drawaxesone
\end{tikzpicture}
\subcaption{}
\end{subfigure}
\caption{(a) Consider small $\epsilon >0$. The lex-value of this game equals $(0.5,1)$ in all three states $s_0, s_1, s_2$. (b) todo}
\label{fig:robust}
\end{figure}

\begin{example}
	\label{ex:}
	In the game in Figure \ref{fig:robust}, the lex-value is $(0.5,1)$ which is for example attained by the strategy of $\plmax$ that goes to the left. However, if $\plmin$ chooses to go to the left in $s_1$ (instead of down, as a lex-optimal counter-strategy would do), we have $\prob^\bothstrats_{s_0}(\objvec) = (0.5+\epsilon,0)$.
\end{example}

Such behavior can be problematic in some practical applications. The goal of this section is to mitigate the problem by providing stronger guarantees about the values $\lexval_i(s)$, $i > 1$.

We will restrict our discussion to $n=2$ objectives for the sake of simplicity. However, all notions can be extended to $n>2$ as well. We will also fix one initial state $\sinit \in S$ of interest. 

\begin{definition}[Justifiable counter-strategy]
	Let $\maxstrat \in \maxstrats$ be lex-optimal. A strategy $\minstrat \in \minstrats$ is called \emphdef{justifiable} if $\prob_\sinit^\bothstrats(\obj_2) < \lexval_{2}(\sinit)$.
\end{definition}

\begin{example}
	Suppose that $\maxstrat$ is a lex-optimal strategy of $\plmax$ in the game from Figure \ref{fig:running_example}. The only justifiable counter-stratgies of $\plmin$ are those that randomize between actions $a$ and $b$ in state $s_1$ because they achieve a value smaller than $\lexval_2(s_1)$ for $\obj_2$. In the game in Figure \ref{fig:robust}, all sub-optimal strategies of $\plmin$ are justifiable.
\end{example}

\subsection{The Coefficient of Robustness}



\begin{definition}[Coefficient of robustness]
	Let $\maxstrat \in \maxstrats$ be lex-optimal. Define the set
	\[
		\Gamma_\maxstrat = \left\{ \gamma \in \R_{\geq 0} \mid \exists \minstrat \in \minstrats \colon \minstrat \text{ is justifiable and } \frac{\prob^\bothstrats_\sinit(\obj_1) - \lexval_{1}(\sinit)}{\lexval_{2}(\sinit) - \prob^\bothstrats_\sinit(\obj_2)} \geq \gamma \right\}.
	\]
	The \emphdef{coefficient of robustness} $\gamma_\maxstrat$ of strategy $\maxstrat$ is defined as $\gamma_\maxstrat = \inf \Gamma_\maxstrat$ (with the convention that  $\inf \emptyset = \infty$).
\end{definition}

With a straightforward calculation, we can show that following:

\begin{proposition}
	For any given lex-optimal $\maxstrat \in \maxstrats$, we have $\gamma_\maxstrat > 0$ and the following assertion holds:
	
	If for some counter-strategy $\minstrat$, we only have $\prob_{\sinit}^\bothstrats(\obj_2) = \lexval_{2}(\sinit) - \delta$, then this implies $\prob_{\sinit}^\bothstrats(\obj_1) \geq \lexval_{1}(\sinit) + \gamma_\maxstrat \delta$.
	
\end{proposition}
%\begin{proof}
%	If $\plmin$ does not have any justifiable counter-strategies, then $\gamma_\sigma=\infty > 0$. Else if there is at least one justifiable counter-strategy
%	To see that $\gamma_\maxstrat > 0$The rest follows by a simple calculation.
%\end{proof}

Thus the decrease by $\delta$ in the secondary objective entails an increase by (at least) $\gamma_\maxstrat \delta$ in the primary objective. In other words, the greater the value $\gamma_\maxstrat$, the more \emph{robust} is $\maxstrat$ against sub-optimal counter-strategies.

\begin{example}
	In the example in Figure \ref{fig:robust}, for strategy $\maxstrat_1$ that chooses $s_1$ we have $\gamma_{\maxstrat_1}=\epsilon$ and for strategy $\maxstrat_2$ choosing $s_2$ it holds that $\gamma_{\maxstrat_2}=1$. Note that in particular, different lex-optimal strategies may have a different coefficient of robustness.
	
\end{example}

\subsection{Computation of $\gamma_\maxstrat$}

\begin{proposition}
	Let $\maxstrat \in \maxstratsmd$ be lex-optimal.
	Let $\alpha$ be the slope of the line segment adjacent to $\lexval(s_0)$ in the Pareto curve of $\objvec$ in the induced MDP $\game^\maxstrat$.
	Then $\gamma_\sigma = -\frac{1}{\alpha}$. In particular $\gamma_\sigma > 0$. 
	
\end{proposition}


\subsection{Approximate Lexicographic Optimization}

\todo[inline]{This is a new, more practically motivated idea. One could simply apply the algorithm but only solve approximately instead of exactly. We are not able to give any guarantees with respect to the real lex-value a priori, but we can compute the coefficient of robustness and then decide based on that if the strategy is good enough.}
